Inertial Asynchronous Computation

Computation is the controlled evolution of a state. Asynchronous evolutions, where all parts of the state change in their own time without stopping each other, put this control in jeopardy. It is in fact a mystery how natural processes perform asynchronous computations using many units with no global orchestration. Here we demonstrate how collective computational abilities can emerge in asynchronous many-body systems. The key insight is to split the physical "hardware" underlying the computation into two asymmetrically coupled parts, analogous to position and momentum in a harmonic oscillator. The resulting inertia nudges the evolution of the state so that the asynchronous computation proceeds in the right order. By treating our inertial asynchronous computer as a nonequilibrium material, we map out its phase diagram numerically and analytically using a framework we dub loop dynamical mean-field theory. We experimentally demonstrate our approach using analog spiking neuromorphic chips designed to mimic actual neurons in the brain. In addition, we construct software that can run on asynchronous hardware: we denoise movies whose clean versions were never seen during training, an instantiation of the generalization transition underlying modern machine learning. Our results point to a general strategy for reliable, decentralized computation in energy-constrained settings from dynamics self-assembly to cell differentiation.

==> latexmkrc <==
# latexmkrc — make the live xr-hyper cross-references between the two
# independent documents resolve on Overleaf.
#
# main.tex and supplement_standalone.tex each \externaldocument the other, so
# each needs the OTHER document's .aux (its \newlabel table) at compile time.
# Overleaf compiles only one "Main document" per run, so when it builds one of
# them the other's .aux may be missing and the cross-references come out as "??".
#
# Fix: before latexmk builds whichever document you asked for, generate BOTH
# .aux files with a fast draft-mode pdflatex pass (draft mode skips images/PDF
# output but still writes every \newlabel).  \externaldocument then always finds
# the other document's labels.  No reference numbers are stored in any .tex file
# — the \ref's stay fully live and auto-update.
#
# Notes:
#  * Assumes the pdflatex engine (revtex4-2's default, and what this project
#    uses).  If you switch the project to xelatex/lualatex, change "pdflatex"
#    below to match.
#  * On Overleaf just set the "Main document" to main.tex or to
#    supplement_standalone.tex and compile as usual; this runs automatically.
foreach my $d ('main', 'supplement_standalone') {
    if (-e "$d.tex") {
        system("pdflatex -interaction=nonstopmode -draftmode \"$d.tex\" > /dev/null 2>&1");
    }
}


==> preamble.tex <==
% Shared preamble for the standalone SI (copied from main.tex lines 2-66).
% Keep in sync with main.tex's preamble if you change packages/macros there.


% Language setting
\usepackage[english]{babel}

% Set page size and margins
% Replace `letterpaper' with `a4paper' for UK/EU standard size
\usepackage[letterpaper,top=2cm,bottom=2cm,left=1.75cm,right=1.75cm,marginparwidth=1.75cm]{geometry}

\usepackage{etoolbox}
\usepackage{titletoc}   % SI-only (partial) table of contents
\AtBeginEnvironment{appendix}{\onecolumn}

% Useful packages
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{csquotes}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks=true, allcolors=OliveGreen]{hyperref}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage[capitalize]{cleveref}


%%%%%%%%%%%%%%%%
%%% symbols %%%
%%%%%%%%%%%%%%%%
\usepackage{amsfonts}
\usepackage{bm}
\newcommand{\dd}{\text{d}}
\newcommand{\DD}{\text{D}}

\newcommand{\ii}{\mathrm{i}}
\newcommand{\Tr}{\mathrm{Tr}}

\def\acursed#1{#1}

%%%%%%%%%%%%%%%%
%%% acronyms %%%
%%%%%%%%%%%%%%%%
\usepackage{acronym}

% Hopfield network
\newacro{HN}{Hopfield network\acused{HN-ad}}
\newacroindefinite{HN}{a}{a}
\newacro{HN-ad}[HN]{Hopfield-network\acused{HN}}
\newacroindefinite{HN-ad}{a}{a}

% mutual information
\newacro{MI}{mutual information\acused{MI-ad}}
\newacroindefinite{MI}{an}{a}
\newacro{MI-ad}[MI]{mutual-information\acused{MI}}
\newacroindefinite{MI-ad}{an}{a}

\def\figurename{Fig.}
\makeatletter
\def\fnum@figure{\textbf{\figurename~\thefigure}}
\makeatother

\usepackage{hyperref}
\usepackage{bookmark}


\newcommand{\gi}[1]{\textcolor{red}{{\bf GI:}~#1}}


